Baryon spectrum of SU(4) composite Higgs theory with two distinct fermion representations

We use lattice simulations to compute the baryon spectrum of SU(4) lattice gauge theory coupled to dynamical fermions in the fundamental and two-index antisymmetric (sextet) representations simultaneously. This model is closely related to a composite Higgs model in which the chimera baryon made up of fermions from both representations plays the role of a composite top-quark partner. The dependence of the baryon masses on each underlying fermion mass is found to be generally consistent with a quark-model description and large-Nc scaling. We combine our numerical results with experimental bounds on the scale of the new strong sector to derive a lower bound on the mass of the top partner.

==> tables/empty_table.tex <==
\begin{tabular}{clllllc}
\toprule

\hline
% Data goes here...
\toprule
\end{tabular}
